Learning Accurate Whole-body Throwing with High-frequency Residual Policy and Pullback Tube Acceleration

Throwing is a fundamental skill that enables robots to manipulate objects in ways that extend beyond the reach of their arms. We present a control framework that combines learning and model-based control for prehensile whole-body throwing with legged mobile manipulators. Our framework consists of three components: a nominal tracking policy for the end-effector, a high-frequency residual policy to enhance tracking accuracy, and an optimization-based module to improve end-effector acceleration control. The proposed controller achieved the average of 0.28 m landing error when throwing at targets located 6 m away. Furthermore, in a comparative study with university students, the system achieved a velocity tracking error of 0.398 m/s and a success rate of 56.8%, hitting small targets randomly placed at distances of 3-5 m while throwing at a specified speed of 6 m/s. In contrast, humans have a success rate of only 15.2%. This work provides an early demonstration of prehensile throwing with quantified accuracy on hardware, contributing to progress in dynamic whole-body manipulation.

==> figures/swing_hw/swing_hw.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{figures/swing_hw/swing_hw1.pdf}
    \caption{\textbf{EE velocity tracking improvement with the residual policy on the hardware.} This figure compares the velocity tracking performance of the control system with and without the residual policy across various commanded end-effector velocities during throws. The improvement from the residual policy is more effective at higher velocities.}
    \label{fig:swing_hw}
    
    % \vspace{1.5cm}
\end{figure}


==> figures/swing_sim/swing_sim.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{figures/swing_sim/swing_sim1.pdf}
    \caption{\textbf{Comparison of residual policies with various frequencies in simulation.} We evaluate the effectiveness of residual policies of various frequencies in reducing EE velocity tracking errors. While all tested frequencies demonstrate improvements over the baseline, the 400 Hz residual policy consistently achieves the best performance.}
    \label{fig:swing_sim}
    
    % \vspace{1.5cm}
\end{figure}

